A Gentle Overview of Asynchronous Session-based Concurrency: Deadlock Freedom by Typing

While formal models of concurrency tend to focus on synchronous communication, asynchronous communication is relevant in practice. In this paper, we will discuss asynchronous communication in the context of session-based concurrency, the model of computation in which session types specify the structure of the two-party protocols implemented by the channels of a communicating process. We overview recent work on addressing the challenge of ensuring the deadlock-freedom property for message-passing processes that communicate asynchronously in cyclic process networks governed by session types. We offer a gradual presentation of three typed process frameworks and outline how they may be used to guarantee deadlock freedom for a concurrent functional language with sessions.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{C. Aubert, C. Di Giusto, S. Fowler \& V. K. I Pun (Eds.):\\
17th Interaction and Concurrency Experience (ICE 2024)\\
EPTCS 414, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.414.1}{10.4204/EPTCS.414.1}}


==> macros.tex <==
\RequirePackage{amsmath}
\RequirePackage{amssymb}

\RequirePackage{xparse}
\RequirePackage{mdframed}
\let\oldfigure\figure
\let\endoldfigure\endfigure
\RenewDocumentEnvironment{figure}{O{} m m}{\oldfigure[#1]\begin{mdframed}}{\end{mdframed}\caption{#2}\label{#3}\endoldfigure}

\def\dashes{\vspace{-.5em}\hbox to \textwidth{\leaders\hbox to 3pt{\hss . \hss}\hfil}\smallskip}
\def\dashline{\rotatebox[origin=c]{90}{$\dabar@\dabar@\dabar@$}}

\DeclareFontShape{T1}{ptm}{m}{scit}{<->ssub * ptm/m/sc}{}
\RequirePackage{xspace}
\def\calculus#1{\textsc{#1}\xspace}
%\def\picalc{\calculus{pi}}
%\def\Picalc{\calculus{Pi}}
\def\picalc{\ensuremath{\pi}\xspace}
\def\Picalc{\ensuremath{\pi}\xspace}
\def\lamcalc{\ensuremath{\lambda}\xspace}
\def\Lamcalc{\ensuremath{\lambda}\xspace}
\def\CP{\calculus{CP}}
\def\AP{\calculus{AP}}
\def\ACP{\calculus{ACP}}
\def\APCP{\calculus{APCP}}
\def\LAST{\calculus{LAST}}
\def\LASTn{\calculus{LAST\textsuperscript{\normalfont n}}}

% `\sepr` for regularly spaced, `\sepr*` for more spacing.
\makeatletter
\def\sepr{\@ifstar\@seprstar\@seprnostar}
\def\@seprnostar{\mathbin{\mbox{\large{$\mid$}}}}
\def\@seprstar{~~\@seprnostar~}
\makeatother

\RequirePackage{mathpartir}
\def\@nonitbrack#1#2{{\normalfont{#1[#2]}}}
\NewDocumentCommand\ruleLabel{s O{} m O{}}{%
    \@nonitbrack{#2}{\textsc{#3}\IfBooleanT{#1}{-\ensuremath{\ast}}}\textsuperscript{#4}%
}
\def\tinyRL#1{{\scriptstyle\ruleLabel{#1}}}
\def\inferLabel#1{\mbox{\scriptsize\normalfont{\ruleLabel{#1}}}}
\NewDocumentCommand\bussRL{O{}}{%
    \IfValueT{#1}{%
        \RightLabel{\scriptsize #1}
    }
}
\RequirePackage{bussproofs}
\NewDocumentCommand\bussAx{O{} m}{\AxiomC{}\bussRL[#1]\UnaryInfC{\ensuremath{#2}}}
\def\bussAssume#1{\AxiomC{\ensuremath{#1}}}
\NewDocumentCommand\bussUn{O{} m}{\bussRL[#1]\UnaryInfC{\ensuremath{#2}}}
\NewDocumentCommand\bussBin{O{} m}{\bussRL[#1]\BinaryInfC{\ensuremath{#2}}}
\NewDocumentCommand\bussTern{O{} m}{\bussRL[#1]\TrinaryInfC{\ensuremath{#2}}}
\NewDocumentCommand\bussQuatern{O{} m}{\bussRL[#1]\QuaternaryInfC{\ensuremath{#2}}}
\def\bussDisplay{\DisplayProof}
\NewDocumentEnvironment{bussproof}{o D(){b}}{%
    \begin{array}[#2]{@{}l@{}}
        \IfValueT{#1}{%
            \inferLabel{#1}
            \\
        }%
        \bottomAlignProof
}{%
        \bussDisplay%
    \end{array}
}
\def\rLbl #1>#2:#3{#1 \rangle #2 : #3}

\let\ol\overline
\def\deq{\mathrel{\triangleq}}
\def\etal{\emph{et al.}\xspace}
\def\<{\langle}
\def\>{\rangle}
\def\lbracket{[}
\def\rbracket{]}

\PassOptionsToPackage{dvipsnames,rgb}{xcolor}
\RequirePackage{xcolor}
\colorlet{cProc}{black}
\colorlet{cType}{RoyalBlue}
\colorlet{cPri}{RedOrange}
\colorlet{cFunc}{YellowOrange}
\def\fProc#1{\textcolor{cProc}{\mathit{#1}}}
\def\fType#1{\textcolor{cType}{\mathsf{#1}}}
\def\fPri#1{\textcolor{cPri}{\mathit{#1}}}
\def\fFunc#1{\textcolor{cFunc}{\mathrm{#1}}}
\def\fCtx#1{\mathcal{#1}}

\RequirePackage{graphicx}
\makeatletter
\def\@rot#1#2{\rotatebox[origin=c]{180}{$#1{#2}$}}
\def\@rott#1{\mathpalette\@rot{#1}}
\makeatother

\RequirePackage{centernot}
\makeatletter
\def\@pOutNoStar #1[#2]{#1[#2]}
\def\@pOutStar #1[#2]{\ol{#1}[#2]}
\def\pOut{\@ifstar\@pOutStar\@pOutNoStar}
\def\pIn #1(#2){#1(#2)}
\def\pRes #1{(\nu #1)}
\def\pResN{\pRes{\_\_}}
\def\@pSelNoStar #1[#2] < #3{#1[#2] \triangleleft #3}
\def\@pSelStar #1 < #2{\ol{#1} \triangleleft #2}
\def\pSel{\@ifstar\@pSelStar\@pSelNoStar}
\def\@pBraNoStar #1(#2) > #3{#1(#2) \triangleright #3}
\def\@pBraStar #1 > #2{#1 \triangleright #2}
\def\pBra{\@ifstar\@pBraStar\@pBraNoStar}
\let\prl\parallel
\def\|{\mathbin{|}}
\def\pFwd [#1<>#2]{[#1 \leftrightarrow #2]}
\def\pClose #1[]{#1[]}
\def\pWait #1(){#1()}
\def\pSub#1{\{#1\}}
\def\alpheq{\mathrel{\fProc{\equiv_\alpha}}}
\def\sc{\mathrel{\fProc{\equiv}}}
\def\scCut{\mathrel{\fProc{{}^{\mathtt{C}}{\equiv}}}}
\def\@reddSymb{\longrightarrow}
\def\@reddNoStar{\mathrel{\fProc{\@reddSymb}}}
\def\@reddStar{\mathrel{\fProc{\@reddSymb^\ast}}}
\def\redd{\@ifstar\@reddStar\@reddNoStar}
\DeclareMathOperator\nredd{\fProc{\centernot\@reddSymb}}
\def\reddCut{\mathrel{\fProc{{}^{\mathtt{C}}\mkern-3mu{\@reddSymb}}}}
\DeclareMathOperator\nreddCut{\fProc{\mkern3mu{}^{\mathtt{C}}\mkern-3mu{\centernot\@reddSymb}}}
\def\comm{\mathrel{\fProc{\rightsquigarrow}}}
\makeatother

\makeatletter
\def\sfAmp{\ensuremath{\text{\textup{\sffamily\&}}}}
\def\parr{\mathbin{\@rott{\sfAmp}}}
\def\with{\sfAmp}
\def\tensor{\mathbin{\otimes}}
\def\lolli{\mathbin{\multimap}}
\def\excl{{!}}
\def\ques{{?}}
\def\tEmpty{\varnothing}
\def\tAP{\mathrel{\vdash}}
\def\tACP{\mathrel{{}^{\mathtt{C}}{\vdash}}}
\def\tAPCP{\mathrel{{}^{\mathtt{P}}{\vdash}}}
\makeatother

\makeatletter
\DeclareFontEncoding{LS2}{}{\noaccents@}
\DeclareFontSubstitution{LS2}{stix}{m}{n}
\DeclareSymbolFont{stix@largesymbols}{LS2}{stixex}{m}{n}
\SetSymbolFont{stix@largesymbols}{bold}{LS2}{stixex}{b}{n}
\DeclareMathDelimiter{\lBrace}{\mathopen}{stix@largesymbols}{"E8}{stix@largesymbols}{"0E}
\DeclareMathDelimiter{\rBrace}{\mathclose}{stix@largesymbols}{"E9}{stix@largesymbols}{"0F}
\makeatother

\makeatletter
\RequirePackage{upgreek}
\def\tAbs{\uplambda}
\def\tOp#1{\mathinner{#1}}
\def\@tSendNoStar #1 #2{\@tSendStar #1 \, #2}
\def\@tSendStar{\tOp{send}}
\def\tSend{\@ifstar\@tSendStar\@tSendNoStar}
\def\tRecv{\tOp{recv}}
\def\tClose{\tOp{close}}
\def\tNew{\tOp{new}}
\def\tFork{\tOp{fork}}
\def\tLet{\tOp{let}}
\def\tIn{\tOp{in}}
\def\@tSelNoStar #1 #2{\@tSelStar #1 \, #2}
\def\@tSelStar{\tOp{sel}}
\def\tSel{\@ifstar\@tSelStar\@tSelNoStar}
\def\tCase{\tOp{case}}
\def\tOf{\tOp{of}}
\def\tSub#1{\lBrace #1 \rBrace}
\def\tHole{[\cdot]}
\def\tMark{\tOp{\upphi}}
\def\tMain{\tOp{\blacklozenge}}
\def\tChild{\tOp{\lozenge}}
\def\tBfr#1{\lbracket #1 \>}
\def\tBfrEmpty{\upepsilon}
\def\tNil{\square}
\def\tEnd{{end}}
\def\scM{\mathrel{\fFunc{{}^{\mathtt{M}}{\equiv}}}}
\def\scC{\mathrel{\fFunc{{}^{\mathtt{C}}{\equiv}}}}
\def\reddM{\mathrel{\fFunc{{}^{\mathtt{M}}\mkern-3mu{\@reddSymb}}}}
\def\@reddCNoStar{\mathrel{\fFunc{{}^{\mathtt{C}}\mkern-3mu{\@reddSymb}}}}
\def\@reddCStar{\mathrel{\fFunc{{}^{\mathtt{C}}\mkern-3mu{\@reddSymb^\ast}}}}
\def\reddC{\@ifstar\@reddCStar\@reddCNoStar}
\DeclareMathOperator\nreddC{\fFunc{{}^{\mathtt{C}}\mkern-3mu{\centernot\@reddSymb}}}
\def\tM{\mathrel{{}^{\mathtt{M}}{\vdash}}}
\def\tB{\mathrel{{}^{\mathtt{B}}{\vdash}}}
\def\tBTo{\mathrel{\>}}
\def\tC#1{\mathrel{{}^{\mathtt{C}}{\vdash^{\fFunc{#1}}}}}
\def\tCMain{\tC{\mkern-3mu{\tMain}}}
\def\tCChild{\tC{\mkern-3mu{\tChild}}}
\makeatother

\def\transConfProc#1#2{{\llbracket #2 \rrbracket_{#1}}}
\def\transBufProc#1#2#3{\transConfProc{#1 \tBTo #2}{#3}}
\let\transTermProc\transConfProc
\def\transType#1{{\llbracket #1 \rrbracket}}
\def\transTypeDual#1{{\llparenthesis #1 \rrparenthesis}}
\def\Boudol#1{\transConfProc{\texttt{B}}{#1}}
\def\HondaT#1{\transConfProc{\texttt{HT}}{#1}}
% \newcommand{\Boudol}[1]{\llbracket #1 \rrbracket_\mathrm{B}}
% \newcommand{\HondaT}[1]{\llbracket #1 \rrbracket_\mathrm{HT}}

\DeclareMathOperator\fn{fn}
\DeclareMathOperator\bn{bn}
\DeclareMathOperator\fv{fv}
\DeclareMathOperator\dom{dom}
\DeclareMathOperator\pr{\textit{pr}}
\DeclareMathOperator\bmin{\textit{min}}

\RequirePackage{tikz}
\usetikzlibrary{tikzmark}

\usetikzlibrary{calc}
\tikzset{
    ncbar angle/.initial=90,
    ncbar/.style={
        to path=(\tikztostart)
        -- ($(\tikztostart)!#1!\pgfkeysvalueof{/tikz/ncbar angle}:(\tikztotarget)$)
        -- ($(\tikztotarget)!($(\tikztostart)!#1!\pgfkeysvalueof{/tikz/ncbar angle}:(\tikztotarget)$)!\pgfkeysvalueof{/tikz/ncbar angle}:(\tikztostart)$)
        -- (\tikztotarget)
    },
    ncbar/.default=0.5cm,
}
\tikzset{square left brace/.style={ncbar=0.1cm}}
\tikzset{square right brace/.style={ncbar=-0.5cm}}

\newcounter{qcounter}
\NewDocumentCommand\q{O{1}}{%
    \setcounter{qcounter}{0}%
    \loop
        \quad%
        \stepcounter{qcounter}%
    \ifnum\value{qcounter}<#1
    \repeat
}

\RequirePackage{mathtools}
\RequirePackage{comment}

